Ditto in the House: Building Articulation Models of Indoor Scenes through Interactive Perception

Virtualizing the physical world into virtual models has been a critical technique for robot navigation and planning in the real world. To foster manipulation with articulated objects in everyday life, this work explores building articulation models of indoor scenes through a robot's purposeful interactions in these scenes. Prior work on articulation reasoning primarily focuses on siloed objects of limited categories. To extend to room-scale environments, the robot has to efficiently and effectively explore a large-scale 3D space, locate articulated objects, and infer their articulations. We introduce an interactive perception approach to this task. Our approach, named Ditto in the House, discovers possible articulated objects through affordance prediction, interacts with these objects to produce articulated motions, and infers the articulation properties from the visual observations before and after each interaction. It tightly couples affordance prediction and articulation inference to improve both tasks. We demonstrate the effectiveness of our approach in both simulation and real-world scenes. Code and additional results are available at https://ut-austin-rpl.github.io/HouseDitto/

==> sections/intro.tex <==
\section{Introduction}

Training on physical hardware has been recognized to be notoriously expensive by the embodied AI and robotic communities~\cite{}. While real-world experiments are time-consuming, unscalable, and hard to reproduce, virtual platforms and synthetic datasets~\cite{} provide a massive amount of affordable training data and a highly-controllable environment.
% Due to the data-hungry nature of AI models, people tend to utilize virtual platforms and synthetic datasets~\cite{} since they provide a massive amount of affordable training data. 
% and enable us to conduct training in a low-cost fashion.
%
Nonetheless, the distribution mismatch between the real and virtual worlds hinders the generalization of models trained in simulation.
% Thus, the realism preserved in the virtual environment is crucial for the applicability.
%

One straightforward path toward closing the reality gap is digitizing and recreating the physical scene in virtual environments. These digital twins are expected to not only be geometrically accurate but also maintain the kinematic relations between the object parts. By leveraging them, the robot can practice the essential skills of localizing and manipulating objects in simulation and validate their performances prior to real-world execution.
% Assume that a robot is deployed in a novel household scene and tasked with daily chores. The robot is expected to learn about the objects in the home and build models of them from its exploratory interactions and the resultant sensory stimuli. These models can, in turn, be used by the robot to practice the essential skills of localizing and manipulating these objects in simulation and validate their performances prior to real-world execution.
%

Latest virtual AI platforms~\cite{} have supported several interactive household scenes, such as kitchen and bedroom, and provided a wide range of carefully-curated articulated objects that can be interacted with virtual agents. However, they heavily rely on human experts to manually curate object assets and scene layouts~\cite{}. The prohibitively high costs of human effort obstruct the broader applicability and scalability of these techniques for simulating diverse real-world scenes.
%
Meanwhile, recent advances in SLAM and 3D vision techniques~\cite{} have empowered mobile agents to construct high-fidelity maps of the real world with minimum human engagement. Yet, the challenge of robot manipulation requires us to move beyond conventional SLAM techniques for building static 3D maps of objects and environments. Rather, we will have to build interactive 3D models that inform the robot’s physical interactions with the objects. 
%


\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figs/teaser.pdf}
    \vspace{-5mm}
    \caption{
    \textbf{Teaser.} \todo{}}
    \label{fig: teaser}
\end{figure}


Despite its importance, building digital twins of interactive scenes has not been systemically studied. \todo{related work}
% nor did that necessarily involve physical interaction with articulated objects or enable the recreation of the full-fledged virtual objects 
%

% Inspired by how children make contact and learn from the physical world through playful activities~\cite{}, we argue that the robot can also learn the properties of physical objects from its own exploratory interactions and the resultant sensory stimuli.
% the interaction with physical objects produces streams of sensorimotor experiences that reveal strong cues to understanding the properties of physical objects. 
% That is, the robot can learn about the objects in the home and build models of them from its exploratory interactions and the resultant sensory stimuli. 
To learn about the objects in the scene and build models of them, the robot needs to know \textit{where} are the actionable regions in an environment, and \textit{how} to infer the articulation model by observing the changes in object state.

% \textit{how} to move the object in order for successful interaction, 
% That is, the two essential ingredients are the scene affordance and the physical articulation model.
% That is, the embodied agents and robots can infer scene geometry and part-level kinematic constraints,~\eg, prismatic or revolute joints, through informative interaction.

Sensing affordance in a novel scene without any prior knowledge is not a trivial task. Existing works infer affordance for tasks such as object grasping~\cite{} where the scene is less cluttered and all objects are actionable. On the other hand, in our work, the agent must deal with a much more complex scene that is filled with non-actionable objects such as sinks or toilets and actionable objects with different underlying kinematic structures such as revolute or prismatic joints.
%
Moreover, reasoning about the kinematic structure is another grand challenge. Inferring the articulation model highly relies on the interior structure of objects, which is often hidden before eligible interaction attempts.
%
As the result, obtaining a reliable affordance and an accurate articulation of all objects in the scene is often unrealistic based only on the initial observation.

% \todo{the hardship of the task}
% Affordance
% 1. non-interactable object
% 2. affordance area
% 3. no prior - cite visual affordance paper

% art
% 1. interior
% 2. clutter scene - where to focus

% Given a novel scene without any prior, it is not trivial to infer the affordance area. Without knowledge of the underlying kinematic structure, the estimation of affordance is ambiguous. For the revolute joint, the affordance only falls in places where the maximum tangent force occurs around the axis. On contrary, the affordance on a prismatic joint may spread on the mobile part surface as long as it moves along the axis.
% Given a novel scene without knowing any underlying kinematic constraint, the estimation of affordance is a challenging task.
% For the revolute joint, the affordance occurs in the region that can maximize the tangent force rotating around the axis. As for the prismatic joint, it must move along the prismatic axis.
% could occur in several different regions and forms of strategy upon the objects. 
%
% \todo{Although the affordance can be directly derived from the articulation model}, reasoning about the kinematic structure is another grand challenge in the absence of observations of the object's interior structure, which can only be exposed after eligible interaction attempts.
%

Our key intuition is that while affordance is highly correlated to the articulation properties of the object, the estimation of the articulation model reversely relies on the views captured after the affordance-based interaction. By leveraging the synergistic relations between affordance and articulation understanding, the robot is able to build simulation models of real-world environments with minimal human supervision even when the initial guess is not fully accurate. 


% Our key intuition is that \todo{while the robot can easily infer affordance from the articulation properties of the object}, the articulation estimation reversely relies on the views captured after the affordance-based interaction. By leveraging the synergistic relations between affordance and articulation understanding, the robot is able to build simulation models of real-world environments with minimal human supervision. 
%
% Due to the occlusion, the interior object parts such as drawers remain unobserved in initial observations. While they can provide helpful clues for articulation estimation, they would only be available until a successful interaction,  which highly relies on a good affordance estimation. 
% Even more, the interior object parts, such as cabinets and drawers, are often occluded in initial observations. They would only be exposed until a successful interaction which highly relies on a good affordance estimation.
% On top of these, we explore the synergistic relations between affordance and articulation model understanding...
%

To realize the above vision, we introduce {XXXX} -- an interactive learning framework that constructs structured virtual object models from a robot’s interactive perception of physical world objects. As shown in~Figure~\ref{fig: teaser}. We leverage PointNet++~\cite{} which takes the static scene point cloud as input and estimates the affordance value of each location. 
%Note that the static scene point cloud is assumed to be known since it can be trivially built upon ego-centric observations collected by a robot through modern techniques such as SLAM. 
%
After that, the robot interacts with the objects under the guidance of the high confidence of the affordance. The interaction is simplified by simulating a teleported ball robot that applies a simple set of forces,~\ie, pulling and pushing. Once we acquired the visual observations captured before and after interactions, they are fed along with the affordance into the next module -- a model built upon Ditto~\cite{} that will infer the corresponding joint parameters, joint state, and part-wise segmentation. 
%
To incorporate the synergistic relations between affordance and articulation model understanding, we re-compute the affordance according to the predicted articulation structures. While reliable affordance sources lead to less occluded observations, the model is able to infer more accurate articulation models. Finally, the scene-level digital twins can be built upon by aggregating the articulation models.

We evaluate our approach on the dataset CubiCasa5K~\cite{}. Our results demonstrate that {XXXX} accurately reconstructs scene-level geometry and articulation model without human intervention. Moreover, the study shows the improvement brought by the synergistic relationships between affordance prediction and articulation model estimation. Finally, we apply our method to real-world scenes for recreating interactive digital twins.




% As for training, we colleted ... igibon and teleported  ball robot



% synergistic relations between geometry reasoning and grasp
% learning. Our key intuition is that a learned representation
% capable of reconstructing the 3D scene encodes relevant geometry information for predicting grasp points and vice versa


% infer the geometry and physics of individual object parts and their articulation relations. On top of these, we also explore the synergies between affordance and articulation model understanding. While

% In this work, we introduce 






% for embodied agents and robots, interaction with physical objects produces streams of 
% sensorimotor experiences that reveal strong cues to understanding the properties of physical objects. In 

% Despite its importance, there has been only limited work on building digital twins of interactive scenes. Cite some work
% %
% % Building digital twins of interactive scenes is a grand challenge that has not been systemically explored. It requires a good understanding of both scene geometry and part-level kinematic constraints,~\eg, prismatic or revolute joints. 
% %
% To acquire such models, the robot must tackle the following challenges: 1.) identifying the high affordance area in a novel scene and 2.) inferring the geometry and physics of individual object parts and their articulation relations.


% Inferring joints, kinematic constraints, and the full 3D structure of articulated objects via interaction is a
% complex task that involves tackling a diverse set of challenges







% Inspired by how children make contact and learn from the physical world through playful activities, we divide

% expose kinematic constraints (e.g., prismatic or revolute joints) and observe occluded part geometry



% not only the scene geometry but

% of its overall geometry but the part compositions as well as the kinematic relations between the parts.



% particularly challenging as it requires


% Building digital twins of articulated objects is particularly challenging as it requires not only a good understanding of its overall geometry but the part compositions as well as the kinematic relations between the parts.

% %
% The project aims at building an interactive learning framework that constructs structured object models 
% from a robot’s physical interaction with real-world objects. This new framework will produce interactive 
% digital twins of physical objects and environments that can be instantiated in a simulation engine for 
% training and validating learning-based manipulation algorithms. 



% Recent years, we have seen the emergence of many simulation environments for robotics and
% embodied AI research



% Recent efforts in embodied AI platforms~\cite{}



% Recent efforts in embodied AI platforms~\cite{} have incorporated interactive articulated objects, such as cabinets and drawers, in simulated household environments and employed them for training virtual agents. Even so, they heavily rely on graphics designers and engineers to author and curate the object models, limiting the scalability of the asset acquisition process.







% Building digital twins of articulated objects is particularly challenging as it requires not only a good understanding of its overall geometry but the part compositions as well as the kinematic relations between the parts.
% %
% Recent efforts in embodied AI platforms~\cite{} have incorporated interactive articulated objects, such as cabinets and drawers, in simulated household environments and employed them for training virtual agents. Even so, they heavily rely on graphics designers and engineers to author and curate the object models, limiting the scalability of the asset acquisition process.
% %











% While simulation tools have gained substantial attention in recent years, existing works usually rely on human experts to manually curate object assets and scene layouts~\cite{}. The prohibitively high costs of human curation hinder a broader applicability and scalability of these techniques for simulating diverse real-world scenes.



% 1. SLAM

% howevert, for task like ... requires robot manipulation ...
% interactive object is essential ...

% 2. human effort



% While SLAM and 3D vision techniques [12, 13, 19] have 
% empowered mobile robots to construct high-fidelity maps of the real world with minimum human 
% engagement, the challenge of robot manipulation requires us to move beyond conventional SLAM 
% techniques for building static 3D maps of objects and environments. Rather, we will have to build 
% interactive 3D models that inform the robot’s physical interactions with the objects. 



% The key challenge is the adaptation of predictive models and control programs acquired in simulation


%  in a virtual environment rather than in the real world.


% The key challenge is the distribution mismatch between the real and virtual worlds hinders the generalization of models trained in simulation. 


% The ability to transfer predictive models and control programs acquired in simulation directly to the real world highly relies on 
% The key challenge in combining learning and simulation is the ability to transfer predictive models and control programs acquired in simulation directly to the real world.


% For vision models to benefit from synthetic data, realism is key — the distribution mismatch be-
% tween the real and virtual worlds hinders the generalization
% of models trained in simulation. A promising path towards
% closing the reality gap is digitizing physical objects and
% recreating them in virtual environments.




% %
% While simulation tools have gained substantial attention in recent years, existing works usually rely on human experts to manually curate object assets and scene layouts~\cite{}. The prohibitively high costs of human curation hinder a broader applicability and scalability of these techniques for simulating diverse real-world scenes.
% %













% digital twin importance ...


% On the other hand interaction with physical objects produces streams of 
% sensorimotor experiences that reveal strong cues to understanding the properties of physical objects. In 
% this project, we aim at developing an interactive learning framework that actively and continually builds 
% structured models of the objects from a robot's self-directed play.
% (careful, we don't really have a downstream task)



% The project aims at building an interactive learning framework that constructs structured object models 
% from a robot’s physical interaction with real-world objects. This new framework will produce interactive 
% digital twins of physical objects and environments that can be instantiated in a simulation engine for 
% training and validating learning-based manipulation algorithms. 

 



% Interactive objects in the simulator
% i.e., digital twin of “scenes” and their potential applications


% Reconstruction of the articulated object at room scale is not well-studied
% Require - scene affordance understanding + obj articulation model


% Challenge: no prior about scene
% - Where is object
% - What joint type
% - How to interact

% Synergies between interaction and articulated mdoel (?)

% Technical detail/contribution of our method
% - aff pred
% - interaction -> observation

% - ditto prediction
% - better afford

% - dittp pred

==> sections/intro_v2.tex <==
\section{Introduction}

Training in real physical environments has been recognized to be notoriously expensive by the embodied AI and robotic communities~\cite{james2019sim}. While real-world experiments are time-consuming, unscalable, and hard to reproduce, virtual platforms and synthetic datasets~\cite{tremblay2018deep, li2021igibson,kolve2017ai2,szot2021habitat} provide a massive amount of affordable training data and a highly-controllable environment.
%
Nonetheless, the distribution mismatch between the real and virtual worlds hinders the generalization of models trained in simulation.

One straightforward path toward closing the reality gap is digitizing and recreating the physical scene in virtual environments. These digital twins are expected to not only be geometrically accurate but also maintain the kinematic relations between the object parts. By leveraging them, the robot can practice the essential skills of localizing and manipulating objects in simulation and validate their performance prior to real-world execution.

Recent virtual AI platforms~\cite{li2021igibson,kolve2017ai2,szot2021habitat} have supported several interactive household scenes, such as kitchen and bedroom, and provided a wide range of carefully-curated articulated objects that can be interacted with virtual agents. However, they heavily rely on human experts to manually curate object assets and scene layouts. The prohibitively high costs of human effort limit the broader applicability and scalability of these techniques for simulating diverse real-world scenes.
%
Meanwhile, recent advances in SLAM and 3D vision techniques~\cite{avetisyan2019scan2cad,newcombe2011kinectfusion,newcombe2015dynamicfusion,geiger2011stereoscan,wu2017marrnet} have empowered mobile agents to construct high-fidelity maps of the real world with minimum human engagement. Yet, they can only build static 3D maps of objects and environments while the challenge of robot manipulation requires us to build interactive 3D models that inform the robot’s physical interactions with the objects.


\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figs/teaser_v2.pdf}
    % \vspace{-5mm}
    \caption{
        \textbf{Overview.} 
        Given a physical scene, our framework predicts the grasp points, interacts with the objects, and collects the observations before and after the interactions. After that, the model jointly reconstructs the part-level geometry and articulation model for each object within the scene. Finally, the interactive scene is recreated in virtual environments.
    }
    % \vspace{-5mm}
    \label{fig: teaser}
\end{figure}


\begin{figure*}[t]
    \centering
    \includegraphics[width=\textwidth]{figs/framework_v3.pdf}
    % \vspace{-5mm}    
    \caption{
        \textbf{Framework.} 
        The affordance network takes the static scene point cloud as input and estimates the affordance value at each location. By applying point non-maximum suppression, we extract the potential contact points from the affordance map. Then, the robot interacts with the object based on those contact points. For each interaction, we feed the point cloud observations before and after the interaction into the articulation model network to obtain the articulation estimation. By aggregating the reconstructed articulated objects, we recreate the interactive virtual scenes.
    }
    \label{fig: framework}
\end{figure*}


% Despite its importance, building digital twins of interactive scenes has not been systemically studied. While perceiving and interacting with articulated objects has been an active line of research, recent studies limit their applicability to a single object rather than complex household scenes. Several studies leverage passive observation to estimate~\cite{jain2020screwnet,abbatematteo2019learning} and reconstruct~\cite{mu2021sdf} articulated objects with the help of modern techniques such as geometric deep learning~\cite{kanazawa2018end,omran2018neural,pavlakos2018learning} and implicit neural representations~\cite{deng2020nasa,noguchi2021neural,jiang2022ditto}. To incorporate interactive perception, recent work takes advantage of informative motion created by scripted actions~\cite{sturm2011probabilistic,katz2013interactive,pillai2015learning} or learned policy~\cite{kumar2019estimating,gadre2021act}. All of the above methods are evaluated in monotonous scenes such as tabletop scenarios.
Building digital twins of interactive scenes has not been systemically studied. While perceiving and interacting with articulated objects has been an active line of research, recent studies focus on single object scenarios rather than complex household scenes. Several studies leverage passive observation to estimate~\cite{jain2020screwnet,abbatematteo2019learning} and reconstruct~\cite{mu2021sdf} articulated objects with the help of modern techniques such as geometric deep learning~\cite{kanazawa2018end,omran2018neural,pavlakos2018learning} and implicit neural representations~\cite{deng2020nasa,noguchi2021neural,jiang2022ditto}. To incorporate interactive perception, recent work takes advantage of informative motion created by scripted actions~\cite{sturm2011probabilistic,katz2013interactive,pillai2015learning} or learned policy~\cite{kumar2019estimating,gadre2021act}. All of the above methods lack of ability to infer the affordance and articulated model in complex scenes and thus cannot be applied to the indoor environment.

To learn about the objects in the scene and build models of them, the robot needs to know \textit{where} are the interactable regions in an environment, and \textit{how} to infer the articulation model by observing the changes in object state.
%
Sensing affordance in a novel scene without any prior knowledge is a challenging task. Existing works infer affordance for manipulation tasks such as object grasping~\cite{kokic2017affordance,jiang2021hand,mo2021where2act} where the scene is less cluttered and all objects are assumed to be interactable. On the contrary, in a household scene, the robot must deal with a much more complex environment that is filled with both non-interactable objects such as tables and beds as well as interactable objects. Even more, the interactable objects may have multiple mobile parts with different underlying kinematic structures such as revolute or prismatic joints. 
% Factors like physical collisions and visual occlusions would also account for obstacles in scene affordance estimation.
%
While mobile parts may move along a prismatic axis or rotate around a revolute axis depending on the underlying kinematic joints, it is ambiguous to estimate the affordance region without any priors. The interaction attempt based on inaccurate affordance may only partially open the object, where the interiors remain hidden by occlusions. Given that reasoning about the kinematic structure highly relies on the observation of the interior structure of objects, such an attempt would result in an unreliable estimation of the articulation model.
% Reasoning about the kinematic structure is another grand challenge. Inferring the articulation model highly relies on the observation of the interior geometry structure of objects, which is often hidden by occlusions until an eligible interaction attempts.
%
As the result, the robot is often not able to obtain a reliable affordance and an accurate articulation of all objects in the scene based only on the initial observations.

Our key intuition is that while affordance location highly depends on the articulation properties of the object, reversely the estimation of the articulation model relies on the views captured after the affordance-based interaction. By leveraging the synergistic relations between affordance and articulation understanding, the robot is able to build simulation models of real-world environments even when the initial prediction is not completely reliable.

To this end, we introduce {XXXX} --- a framework that recreates the virtual scenes from a robot’s interactive perception of physical world objects. 
%
As shown in Figure~\ref{fig: teaser}, we first estimate the affordance values at each location and infer the grasp points from them.
%
After that, the robot interacts with the objects according to the inferred grasp points. 
% During training, the interaction is simplified by simulating a teleported ball robot that applies a simple set of forces,~\ie, pulling and pushing. 
Once we acquired the visual observations captured before and after interactions, they are fed along with the affordance into the next module, where the model will infer the corresponding joint parameters, joint state, and part segmentation of each object. 
%
To incorporate the synergistic relations between affordance and articulation model understanding, we re-compute the affordance according to the predicted articulation structures. While more reliable affordance sources lead to less-occluded observations, the model is able to infer more accurate articulation models. Finally, the scene-level interactive model can be built upon by aggregating the reconstructed articulated objects.

We evaluate our approach on the dataset CubiCasa5K~\cite{kalervo2019cubicasa5k} in the iGibson~\cite{li2021igibson} simulator. Our results demonstrate that {XXXX} accurately reconstructs scene-level geometry and articulation model without human intervention. Moreover, the ablation studies confirm the benefits of the exploitation of the synergies between affordance prediction and articulation model estimation. Finally, we apply our method to a physical scene and successfully recreate the corresponding interactive digital twins.




==> sections/intro_v3.tex <==
\section{Introduction}
% Embodied tasks such as interactive navigation~\cite{} and interactive question answering~\cite{} in indoor environments require the robot to navigate and manipulate objects in the scene. In order to achieve the goal, the robot may need to interact with articulated objects such as opening a cabinet. Moreover, emerging 3D applications like augmented reality depend on the ability to sense and interact with the environment in order to overlay digital interactive augmentations. To facilitate these applications, we need a persistent scene representation that not only accurately describes the geometry but also captures the underlying kinematic relations in the environments.
%

% Modern techniques such as SLAM and 3D reconstruction~\cite{avetisyan2019scan2cad,newcombe2011kinectfusion,newcombe2015dynamicfusion,geiger2011stereoscan,wu2017marrnet} have empowered mobile agents to construct high-fidelity maps of the real world with minimum human engagement. However, these maps typically contain geometric information that only covers the static environment. For tasks such as robot manipulation, we would need interactive 3D models that inform the robot’s physical interactions with the objects.
%

% Recent advances in structure sensors and SLAM techniques~\cite{newcombe2011kinectfusion,newcombe2015dynamicfusion,geiger2011stereoscan} have substantially improved the fidelity of reconstructions of real-world scenes.

Manipulation is an essential skill for robots to operate in human environments. Unlike in factories where the objects are usually known as priori, manipulating objects in human environments is challenging due to the variation and diversity of the objects. Human environments are populated with articulated objects, ranging from furniture to small tabletop objects. Effectively manipulating these objects requires a deep understanding of their articulation models. Such understanding is beyond the scope of techniques such as SLAM and 3D reconstruction which only build the static 3D maps of real-world scenes. To facilitate robot manipulation in human environments, we need a persistent articulated model of the scene that not only accurately describes the geometry but also captures the underlying kinematic relations of the articulated objects in the environments. This articulated model informs the robot of available physical interactions with the objects.

% An alternative way is to train the robot in virtual scenes where it can practice the essential skills of localizing and manipulating objects. Recent virtual AI platforms~\cite{li2021igibson,kolve2017ai2,szot2021habitat} have supported several interactive household scenes, such as kitchen and bedroom, and provided a wide range of carefully-curated articulated objects that can be interacted with virtual agents. However, the algorithm trained in the simulator suffers from the distribution mismatch between the real and virtual worlds.


\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figs/teaser_v2.pdf}
    % \vspace{-5mm}
    \caption{
        \textbf{Overview.} 
        Given a physical scene, our framework infers the interaction hotspots from the predicted affordance heatmap. For each interaction hotspot, the robot interacts with the objects and collects the corresponding observations before and after the interactions. After that, the model estimated the articulated model based on the observations. Finally, we build the articulated models of the scene by aggregating the object-level estimated articulation models.
    }
    % \vspace{-5mm}
    \label{fig: teaser}
\end{figure}


\begin{figure*}[t]
    \centering
    \includegraphics[width=\textwidth]{figs/framework_v3.pdf}
    % \vspace{-5mm}    
    \caption{
        \textbf{Framework.} 
        The affordance network takes the static scene point cloud as input and estimates the affordance value at each location. By applying point non-maximum suppression, we extract the interaction hotspots from the affordance map. Then, the robot interacts with the object based on those contact points. For each interaction, we feed the point cloud observations before and after the interaction into the articulation model network to obtain the articulation estimation. By aggregating the reconstructed articulated objects, we build the articulated models of the scene.
    }
    \label{fig: framework}
\end{figure*}

% To extend the static 3D maps with interactive properties, we reconstruct the object geometry along with its kinetic constraints such as prismatic and revolute joints through the interactive perception of the robot. Specifically, the robot needs to know \textit{where} are the interactable regions in an environment, and \textit{how} to infer the articulation model by observing the changes in object state. These two tasks are challenging given no prior knowledge such as the locations and types of the objects within the scene.

Building the articulated model of interactive scenes has not been systemically studied. The closest line of research to our work is the object-level articulated model estimation. Some studies leverage only visual perception to estimate the articulated model with the help of geometric deep learning~\cite{kanazawa2018end,omran2018neural,pavlakos2018learning}, implicit neural representations~\cite{deng2020nasa,noguchi2021neural} and inferred kinematic hierarchy~\cite{hameed2022learning}. Most of these works are either category-dependent or rely on a kinematic template and therefore can not be applied to a complex scene where arbitrary numbers, types, and kinematic constraints of objects are presented. Another line of work incorporates interactive perception during articulated model estimation. They take advantage of informative motion created by scripted actions~\cite{sturm2011probabilistic,katz2013interactive,pillai2015learning,jiang2022ditto} or learned policy~\cite{kumar2019estimating,gadre2021act}. All of the above methods are applied to single object scenarios. Thus, they cannot be adapted to indoor environments where the scene is cluttered and the object's location remains unknown.

To build articulated models of indoor environments, we employ interactive perception to extend the static 3D maps with articulation models. A robot actively interacts with the objects, creates observations of articulated objects in novel states, and reconstructs the object geometry along with its kinetic constraints. The robot needs to know \textit{where} are the interactable regions in an environment and \textit{how} to infer the articulation model by observing the changes in object state. These two tasks are challenging given no prior knowledge such as the locations and types of the objects within the scene.

% To determine the interactable regions, the robot needs to infer the affordance that exists in the scene. Previous works propose to infer affordance for human activities~\cite{fouhey2012people} and interaction hotspots~\cite{nagarajan2019grounded} within an indoor environment. However, these approaches rely on videos that demonstrate how people interact with the environment. While our robot is deployed in a novel scene, such demonstrations would not be available. Another active line of research encourages the robot to actively explore affordance in order to interact with the objects~\cite{mo2021where2act} or scenes~\cite{nagarajan2020learning} by policy learning. While they focus on extensively exploring the affordance existing in an environment, we aim to leverage interactive perception in order to recover the articulated model of an interactive scene.

% Our intuition is that the articulated models may reveal important affordance information. A mobile part that can be moved along a prismatic axis or rotated around a revolute axis has a different affordance distribution. While estimating scene affordance is challenging, the articulation prediction can help refine the initial affordance prediction. Moreover, interactions based on the refined affordance may open the object to a larger degree and reveal more object's interior. Such observation can improve the articulation prediction in return. By leveraging this intuition, we demonstrate that the robot is able to build an accurate articulated model even when the initial predictions are not reliable.

Interactable regions in the scene have high affordance. Existing works propose to learn affordance from human activities~\cite{fouhey2012people,nagarajan2019grounded} or active exploration~\cite{mo2021where2act,nagarajan2020learning}. These works apply the learned model to static observations to predict affordance. Apart from the static observations, articulation models also contain important affordance information since they describe how different parts of the object can move. Therefore, we can use the initial coarse articulation model to infer interaction that leads to more significant state changes and further refine the articulation estimation.

% Existing works infer affordance for manipulation tasks such as object grasping~\cite{kokic2017affordance,jiang2021hand,mo2021where2act} where the scene is less cluttered. On the contrary, in a household scene, the robot must deal with a much more complex environment that is filled with objects with or without articulated structure. Even more, the articulated objects may have multiple mobile parts with different underlying kinematic structures such as revolute or prismatic joints. 
% %
% Given that mobile parts may move along a prismatic axis or rotate around a revolute axis depending on the underlying kinematic joints, the affordance area may distribute in different areas even under similar object shapes. Thus, it is ambiguous to estimate the affordance region without knowing the articulation properties. 


% Our key intuition is that while affordance location highly depends on the articulation properties of the object, reversely the estimation of the articulation model relies on the views captured after the affordance-based interaction. The interaction based on accurate affordance can fully open the object part and reveal its interior, which would benefit the reasoning about the kinematic structure. To address the unreliable initial estimation of affordance and articulation model, we propose to extract part-level affordance information from articulation predictions. Our experiment shows that the extracted affordance region enables us to open the joint to a larger degree and thus results in a more accurate articulation prediction. By leveraging the synergistic relations between affordance and articulation understanding, the robot is able to build articulated models of the physical scene even when the initial prediction is not completely reliable.

To this end, we introduce {XXXX} --- a framework that builds the articulated models of indoor environments.
%
As shown in Figure~\ref{fig: teaser}, our approach aims to find the interactable region and infer the articulated model from the robot's interactive perception. To determine the interactable region, we propose to estimate the affordance values at each location and apply a filtering method to obtain a set of interaction hotspots. For each interaction hotspot, we interact with the object at the corresponding locations. After that, we collect the observation of the object before and after the interaction  to infer the articulated models. 
%
To overcome the challenges posed by unreliable predictions at the initial stage, we propose an iterative process  to refine the predictions. At first, we extract the part-level affordance from estimated articulated models. While more reliable affordance sources lead to less-occluded observations, the model is able to improve the accuracy of the articulation predictions. Finally, we build the articulated models of the scene by aggregating the object-level estimated articulation models.
%

We evaluate our approach on the CubiCasa5K~\cite{kalervo2019cubicasa5k} dataset in the iGibson~\cite{li2021igibson} simulator. Our results demonstrate that {XXXX} accurately recovers \todo{more than $XX\%$ joints under $XX$ average error} within the scenes. Moreover, the ablation studies confirm the effectiveness of the iterative process that improves both the affordance and articulated model estimation. Finally, we apply our method in a real world scenario and successfully build the articulated models of the indoor scene.




==> sections/intro_v4.tex <==
\section{Introduction}

Recent advances in structure sensors and SLAM algorithms~\cite{newcombe2011kinectfusion,newcombe2015dynamicfusion,geiger2011stereoscan} have equipped autonomous robots with the ability to build static maps of real-world environments at unprecedented fidelity. These advances have played an integral role in the widespread deployment of mobile robots and self-driving vehicles. Nonetheless, the lack of robust manipulation capabilities has impeded the success of assistive robots in homes, offices, and hospitals. Manipulation in these everyday environments often involves interacting with articulated objects, such as cabinets and doors. Modeling articulated objects requires robots to depart from reconstructing the geometry of a static scene to understanding the kinematic relations and physics of object parts.

% Reasoning about object articulations has been a long standing challenge in robotics. \yuke{rewrite this paragraph...}
% The closest line of research to our work is the object-level articulated model estimation. Some studies leverage only visual perception to estimate the articulated model with geometric deep learning~\cite{kanazawa2018end,omran2018neural,pavlakos2018learning}, implicit neural representations~\cite{deng2020nasa,noguchi2021neural}  and inferred kinematic hierarchy~\cite{hameed2022learning}. Most of these works are either category-dependent or rely on a kinematic template and therefore can not be applied to a complex scene where arbitrary numbers, types, and kinematic constraints of objects are presented. Another line of work incorporates interactive perception during articulated model estimation. They take advantage of informative motion created by scripted actions~\cite{sturm2011probabilistic,katz2013interactive,pillai2015learning,jiang2022ditto} or learned policy~\cite{kumar2019estimating,gadre2021act}. All of the above methods are applied to single object scenarios. Thus, they cannot be adapted to indoor environments where the scene is cluttered and the object's location remains unknown.

Reasoning about object articulations has been a long standing challenge in robotics. Probabilistic methods~\cite{} are first used to  estimate the articulation models. They usually rely on markers or handcrafted features to track the mobile parts which are not available or accurate in the complex human environments. Recently learning-based models infer articulation model from single raw observations by learning category priors from dataset~\cite{}. These models are limited to category-level prediction and can not generalize to the diverse set of daily objects. Other works~\cite{}, such as Ditto~\cite{jiang2022ditto}, employ interactive perception to estimate articulation. They leverage robot interactions to generate novel visual stimuli and estimate articulation from the change of object states. These works most focus on object-level articulation model estimation. Building room-scale articulated models from these object-level models is non-trivial because the robot needs to actively explore the environment and locate and interact with the articulated objects.


In this work, we aim to enable a robot to build articulated models of an indoor environment through its self-directed exploration in the environment. We develop an interactive perception approach~\cite{}, where a robot physically interacts with articulated objects and infers their articulation properties from visual observations before and after the interactions. This task requires the robot to identify regions of possible articulations in a large-scale 3D space, manipulate the objects to create articulated motions, and infer the underlying kinematic parameters from partial observations. 

The most critical challenge of this interactive perception approach is to determine candidate actions that are most effective for probing the environment, \textit{i.e.}, those most likely to spot articulations. Inspired by where2act~\cite{mo2021where2act}, we learn to identify interactable regions of indoor scenes through agent's embodied explorations. 
% Prior works cast this as an affordance prediction problem and identified interactable regions of indoor scenes as high affordance, with models trained on videos of human activities~\cite{fouhey2012people,nagarajan2019grounded} or the agent's embodied explorations~\cite{mo2021where2act,nagarajan2020learning}. 

% To build articulated models of indoor environments, we employ interactive perception to extend the static 3D maps with articulation models. A robot actively interacts with the objects, creates observations of articulated objects in novel states, and reconstructs the object geometry along with its kinetic constraints. The robot needs to know \textit{where} are the interactable regions in an environment and \textit{how} to infer the articulation model by observing the changes in object state. These two tasks are challenging given no prior knowledge such as the locations and types of the objects within the scene.

% To exert effective actions for probing the environments, our method first 

% To determine the interactable regions, the robot needs to infer the affordance that exists in the scene. Previous works propose to infer affordance for human activities~\cite{fouhey2012people} and interaction hotspots~\cite{nagarajan2019grounded} within an indoor environment. However, these approaches rely on videos that demonstrate how people interact with the environment. While our robot is deployed in a novel scene, such demonstrations would not be available. Another active line of research encourages the robot to actively explore affordance in order to interact with the objects~\cite{mo2021where2act} or scenes~\cite{nagarajan2020learning} by policy learning. While they focus on extensively exploring the affordance existing in an environment, we aim to leverage interactive perception in order to recover the articulated model of an interactive scene.

% Our intuition is that the articulated models may reveal important affordance information. A mobile part that can be moved along a prismatic axis or rotated around a revolute axis has a different affordance distribution. While estimating scene affordance is challenging, the articulation prediction can help refine the initial affordance prediction. Moreover, interactions based on the refined affordance may open the object to a larger degree and reveal more object's interior. Such observation can improve the articulation prediction in return. By leveraging this intuition, we demonstrate that the robot is able to build an accurate articulated model even when the initial predictions are not reliable.

The most critical challenge of this interactive perception approach is to determine candidate actions that are most effective for probing the environment, \textit{i.e.}, those most likely to spot articulations. Prior works cast this as an affordance prediction problem and identified interactable regions of indoor scenes as high affordance, with models trained on \yuke{[what does ``human activities'' mean? human videos?] human activities}~\cite{fouhey2012people,nagarajan2019grounded} or the agent's embodied explorations~\cite{mo2021where2act,nagarajan2020learning}. \yuke{[unclear why this sentence is here? are we saying that we are doing the same thing as them or are we saying we are different in whatever way?] These works apply the learned model to static observations to predict affordance.}
\yuke{[is your insight or observation in others' works? i think you are trying to say something about the synergies, but it is not described clearly] Apart from the static observations, articulation models also contain important affordance information since they describe how different parts of the object can move. Therefore, we can use the initial coarse articulation model to infer interaction that leads to more significant state changes and further refine the articulation estimation.}

% Existing works infer affordance for manipulation tasks such as object grasping~\cite{kokic2017affordance,jiang2021hand,mo2021where2act} where the scene is less cluttered. On the contrary, in a household scene, the robot must deal with a much more complex environment that is filled with objects with or without articulated structure. Even more, the articulated objects may have multiple mobile parts with different underlying kinematic structures such as revolute or prismatic joints. 
% %
% Given that mobile parts may move along a prismatic axis or rotate around a revolute axis depending on the underlying kinematic joints, the affordance area may distribute in different areas even under similar object shapes. Thus, it is ambiguous to estimate the affordance region without knowing the articulation properties. 


% Our key intuition is that while affordance location highly depends on the articulation properties of the object, reversely the estimation of the articulation model relies on the views captured after the affordance-based interaction. The interaction based on accurate affordance can fully open the object part and reveal its interior, which would benefit the reasoning about the kinematic structure. To address the unreliable initial estimation of affordance and articulation model, we propose to extract part-level affordance information from articulation predictions. Our experiment shows that the extracted affordance region enables us to open the joint to a larger degree and thus results in a more accurate articulation prediction. By leveraging the synergistic relations between affordance and articulation understanding, the robot is able to build articulated models of the physical scene even when the initial prediction is not completely reliable.


\yuke{before this paragraph, we should have a few sentences introducing Ditto. so the reviewers do not feel that we are overclaiming when they realize that we build on Ditto} 
To this end, we introduce \textsc{HouseDitto}, an interactive perception approach to building the articulated models of indoor scenes.
%
As shown in Figure~\ref{fig: teaser}, our approach aims to find the \yuke{[how is \textit{interactable region} different from \textit{interactable hotspot}?] interactable regions} and infer the articulated model \yuke{[unclear phrase, what is \textbf{from interactive perception}?] from the robot's interactive perception}. To determine the interactable region, HouseDitto estimates the \yuke{affordance values [\textbf{values} too generic word - be more specific]} at each 3D location \yuke{[what is this? is this important?] and apply a filtering method} to obtain a set of interaction hotspots. For each interaction hotspot, we interact with the object at the corresponding locations. We then collect visual observations of the object before and after the interaction  to infer the articulated models. 
%
To overcome the challenges posed by unreliable predictions at the initial stage, we \yuke{[do not use the word \textbf{propose} by the time you write this paper, the work is (almost) done. say words like \textbf{design}, \textbf{develop}, etc. instead] propose} an iterative procedure to refine our predictions. At first, we extract the part-level affordance from estimated articulated models. While more reliable \yuke{affordance sources [confusing term]} lead to less-occluded observations, the model is able to improve the accuracy of the articulation predictions. Finally, we build the articulated models of the scene \yuke{[meaning of \textbf{aggregating} is unclear] by aggregating the object-level estimated articulation models.}
%

We evaluate our approach on the CubiCasa5K~\cite{kalervo2019cubicasa5k} dataset with the iGibson~\cite{li2021igibson} simulator. Our results demonstrate that {XXXX} accurately recovers \todo{more than $XX\%$ joints under $XX$ average error} within the scenes. Moreover, the ablation studies confirm the effectiveness of the iterative process that improves both the affordance and articulated model estimation. Finally, we apply our method in a real world scenario and successfully build the articulated models of the indoor scene.




==> sections/intro_v5.tex <==
\section{Introduction}


Recent advances in structure sensors and SLAM algorithms~\cite{newcombe2011kinectfusion,newcombe2015dynamicfusion,geiger2011stereoscan} have equipped autonomous robots with the ability to build static maps of real-world environments at unprecedented fidelity. These advances have played an integral role in the widespread deployment of mobile robots and self-driving vehicles. Nonetheless, the lack of robust manipulation capabilities has impeded the success of assistive robots in homes, offices, and hospitals. Manipulation in these everyday environments often involves articulated objects, such as cabinets and doors. Physical interaction with these objects requires a robot to depart from reconstructing a static scene to understanding the kinematics and articulation properties of object parts.

% Probabilistic methods~\cite{dearden2005learning,sturm2008adaptive,sturm2008unsupervised,sturm2009learning} are first used to estimate the articulation models. They usually rely on markers or handcrafted features to track the mobile parts, which are not available or accurate in complex human environments.
Reasoning about object articulations has been a long-standing challenge in robotics. A series of learning-based approaches attempt to infer articulation from single visual observations by training models on large 3D datasets~\cite{li2020category,weng2021captra}. These models typically rely on category-level priors, which limit their generalizations toward daily objects. A parallel thread of research~\cite{hausman2015active,martin2014online} uses interactive perception~\cite{bohg2017interactive}. They leverage physical interactions to produce visual observations of articulated motions from which they estimate the articulation properties. These works primarily focus on individual objects, whereas scaling to room-sized environments requires the robot to efficiently and effectively explore the large-scale 3D space for meaningful interactions.
% In contrast, building room-scale articulated models from these object-level models is non-trivial because the robot needs to actively explore the environment and locate and interact with the articulated objects.

\begin{figure}[t]
    \centering
    % \includegraphics[width=\linewidth]{figs_jpg/teaser_v2.jpg}
    \includegraphics[width=\linewidth]{figs_jpg/teaser_v2_zhenyu.jpg}
    % \includegraphics[width=\linewidth]{figs/teaser_v3.pdf}
    % \vspace{-5mm}
    \caption{
        \textbf{Building scene-level articulated models through interactive perception.} 
        From an initial observation of an indoor scene, our approach infers the interaction hotspots, which guide the robot to interact with articulated objects, and collects the observations before and after the interactions. Based on the observed articulated motions, it builds the articulated models of individual objects and aggregates them into a scene-level articulated model.
    }
    % \vspace{-5mm}
    \label{fig: teaser}
\end{figure}

In this work, we aim to enable a robot to build articulated models of an indoor environment through its self-directed exploration. We develop an interactive perception approach, where the robot discovers and physically interacts with articulated objects and infers their articulation properties from visual observations before and after the actions. It requires the robot to identify regions of possible articulations in a large-scale 3D space, manipulate the objects to create articulated motions, and infer the underlying kinematic parameters from partial observations. 

% interactive perception (how to interact)
The foremost challenge is determining the most effective actions for probing the environment, \textit{i.e.}, those most likely to discover articulations. We cast this problem as inferring \textit{scene affordance} from visual observations~\cite{mo2021where2act,nagarajan2020learning,do2018affordancenet}. Specifically, we train a model to predict affordance based on the robot's past interaction experiences with a large collection of procedurally generated 3D scenes in simulation. Furthermore, we introduce an iterative procedure that uses the initial observations of articulated motions as visual cues to refine the affordance predictions. This refined affordance, in turn, guided the robot's subsequent interactions to obtain more informative observations for articulation inference.

% through the agent's embodied explorations. The agent randomly explores the simulated indoor scenes and interacts with the possible articulated objects. We learn from the interaction history to infer the interaction hotspots, the regions on articulated objects that afford interactions.

% perception-action loop
% We infer the articulation model given the observations created by interacting with the predicted hotspots. The perceived articulation model specifies the movable part of the articulated object, which turns out to be the actionable region. Moreover, interacting with this part can create significant visual stimuli for accurate articulation estimation. By closing this perception-action loop, we can refine the articulation estimation and interaction hotspots prediction alternatively.

% To this end, we introduce an interactive perception approach to building articulated models of indoor scenes.
%
Figure~\ref{fig: teaser} illustrates the high-level steps of our approach. It discovers the interaction hotspots (\emph{i.e.}, promising locations for probing actions), creates observations of articulated motions through action, and infers articulation from the observations. 
%
To locate interaction hotspots, we use an affordance model to predict an affordance map from the point cloud observation of an indoor scene.
% The model is trained on data generated by simulating the agent's exploration and interaction.
%
% It obtains a set of interaction hotspots from the learned visual affordance model. 
At the location of each interaction hotspot, the robot tries interacting with the objects and collects egocentric observations of the object before and after its motion caused by the robot's actions. We build the articulation estimation model based on prior work Ditto~\cite{jiang2022ditto} to infer the object articulation from these observations. The articulation estimation model takes as input the robot's action and the visual observations and predicts the articulation parameters of the objects.
%
To improve the quality of our predictions, we tightly couple the two steps of affordance prediction and articulation inference in an iterative process. We extract part-level affordance from the initial (and possibly inaccurate) estimation of articulated models. The robot interacts with the object following the part-level affordance, creating more visible articulation motions that facilitate articulation inference.

We evaluate our approach on the CubiCasa5K~\cite{kalervo2019cubicasa5k} dataset with the iGibson~\cite{li2021igibson} simulator. Quantitative results demonstrate that our approach successfully discovered around 45\% more parts than our baseline with higher precision. Our approach also gives a 51\% absolute segmentation IoU boost compared with the baseline. Moreover, the ablation studies confirm that the iterative refinement process benefits both affordance prediction and articulated model estimation. Finally, we apply our method to a real-world kitchen scene and successfully build an articulated model of this environment.


==> sections/misc.tex <==

\begin{algorithm}
\caption{Point-wise Non-Maximum Suppression}
\label{alg: NMS}
\begin{algorithmic}[1]

\Require $P=\{p_1,...,p_n\}$, $S=\{s_1,...,s_n\}$, d(.), $t$ \newline
$P$ is the set of points \newline
$S$ is the corresponding affordance score \newline
$d(.)$ is the Euclidean distance function \newline
$t$ is the distance threshold \newline

\State $O \leftarrow \{\}$
\While {$P \neq \emptyset$}
\State $m \leftarrow$ argmax $S$
\State $M \leftarrow P_m$
\State $O \leftarrow O \cup M; P \leftarrow P-M$
\For { $p_i \in P$ }
    \If {$d(p_i, P_m) < t$}
        \State $P \leftarrow P - p_i; S \leftarrow S - s_i$
    \EndIf
\EndFor
\EndWhile
\Ensure {$O$}

\end{algorithmic}
\end{algorithm}

==> sections/qualitative.tex <==
% \begin{table*}[t]
%     \small
%     \centering
%     % \vspace{-3mm}
%     \caption{Quantitative results of affordance estimation.}
%     % \vspace{-4mm}
%     \begin{tabular}{l|l|c|c|ccc}
%     \toprule
% \raisebox{\dimexpr-1\normalbaselineskip-2\cmidrulewidth-2\aboverulesep}[0pt][0pt]{} & \raisebox{\dimexpr-1\normalbaselineskip-2\cmidrulewidth-2\aboverulesep}[0pt][0pt]{Method} & \multicolumn{1}{c|}{Precision} & \multicolumn{4}{c}{Coverage} \\
%       \cmidrule{3-7}
%       & & \raisebox{\dimexpr-1\normalbaselineskip-1\cmidrulewidth-1\aboverulesep}[0pt][0pt] {\shortstack[c]{-}} & Prismatic & \multicolumn{3}{c}{Revoulute} \\
%       \cmidrule{4-7}
%      & & & - & Deg. $>15\degree$ & Deg. $>30\degree$ & Deg. $>45\degree$ \\
     
%      \midrule
%      \multirow{2}{*}{\shortstack[l]{Initial stage}}
%      & 3D-AffordanceNet~\cite{deng20213d} & 0.37 & 0.15 & 0.22 & 0.03 & 0.03 \\
%      & $Ours_{init}$ & 0.61 & 0.60 & 0.68 & 0.07 & 0.06 \\
     
%      \midrule
%      \multirow{2}{*}{\shortstack[l]{Final stage}}
%      & $Ours_{final}$ (Art. only) & - & - & X & X & X \\
%      & $Ours_{final}$ & - & - & 0.68 & 0.65 & 0.61 \\     
     
%      \bottomrule
%     \end{tabular}
%     \label{tab:affordance}
% \end{table*}



\begin{table}[t]
    \small
    \centering
    \begin{tabular}{l|c|c|ccc}
    \toprule
\raisebox{\dimexpr-1\normalbaselineskip-2\cmidrulewidth-2\aboverulesep}[0pt][0pt]{Method} & \multicolumn{1}{c|}{Precision} & \multicolumn{4}{c}{Coverage} \\
      \cmidrule{2-6}
      & \raisebox{\dimexpr-1\normalbaselineskip-1\cmidrulewidth-1\aboverulesep}[0pt][0pt] {\shortstack[c]{-}}  & Prismatic & \multicolumn{3}{c}{Revoulute} \\
      \cmidrule{3-6}
      & & - & Deg. $<15\degree$ & Deg. $<30\degree$ & Deg. $<45\degree$ \\
     \midrule
     3D-AffordanceNet~\cite{} & 0.37 & 0.15 & 0.22 & 0.03 & 0.03 \\
     Ours & 0.61 & 0.60 & 0.68 & 0.07 & 0.06 \\
     Ours (art) & - & - & X & X & X \\
     Ours (art+moment) & - & - & 0.68 & 0.65 & 0.61 \\
     % Ours+art & X & - & X & X \\
     \bottomrule
    \end{tabular}
    % \vspace{-3mm}
    \caption{Quantitative results of affordance estimation.}
    % \vspace{-4mm}
%     \label{tab:affordance}
\end{table}



% \begin{table*}[t]
%     \small
%     \centering
%     % \vspace{-3mm}
%     \caption{Quantitative results of articulation prediction.}
%     % \vspace{-4mm}
%     \begin{tabular}{l|l|c|c|c|cc}
%     \toprule
% \raisebox{\dimexpr-1\normalbaselineskip-2\cmidrulewidth-2\aboverulesep}[0pt][0pt]{} & \raisebox{\dimexpr-1\normalbaselineskip-2\cmidrulewidth-2\aboverulesep}[0pt][0pt]{Method} & \raisebox{\dimexpr-1\normalbaselineskip-2\cmidrulewidth-2\aboverulesep}[0pt][0pt]{w/ Contact region} & \multicolumn{1}{c|}{Geometry} & \multicolumn{3}{c}{Joint} \\
%       \cmidrule{4-7}
%       & & & \raisebox{\dimexpr-1\normalbaselineskip-1\cmidrulewidth-1\aboverulesep}[0pt][0pt] {\shortstack[c]{Mobile \\ Seg. IoU $\uparrow$}}  & Prismatic & \multicolumn{2}{c}{Revoulute} \\
%       \cmidrule{5-7}
%       & & & & Angle Err. $\downarrow$ & Angle Err. $\downarrow$ & Pos Err. $\downarrow$ \\
%      \midrule
%      \multirow{4}{*}{\shortstack[l]{Initial stage}}
%      & ScrewNet~\cite{jain2020screwnet} & - & X & X & X & X \\
%      & ANCSH~\cite{li2020category} & - & X & X & X & X \\     
%      \cmidrule{2-7}
%      & $Ours_{init}$ & $\times$ & 0.69 & 0.05 & 29.26 & 0.05 \\
%      & $Ours_{init}$ & $\checkmark$ & 0.75 & 0.04 & 28.70 & 0.05 \\
%      \midrule
%      \multirow{2}{*}{\shortstack[l]{Final stage}}
%      & $Ours_{final}$ (Art. only) & $\checkmark$ & X & - & X & X \\
%      & $Ours_{final}$ & $\checkmark$ & 0.81 & - & 13.50 & 0.02 \\
%      \bottomrule
%     \end{tabular}
%     \label{tab:articulation}
% \end{table*}



% \begin{table*}[t]
%     \small
%     \centering
%     % \vspace{-3mm}
%     \caption{Quantitative results of articulation prediction.}
%     % \vspace{-4mm}
%     \begin{tabular}{l|l|c|c|cc}
%     \toprule
% \raisebox{\dimexpr-1\normalbaselineskip-2\cmidrulewidth-2\aboverulesep}[0pt][0pt]{} & \raisebox{\dimexpr-1\normalbaselineskip-2\cmidrulewidth-2\aboverulesep}[0pt][0pt]{Method} & \multicolumn{1}{c|}{Geometry} & \multicolumn{3}{c}{Joint} \\
%       \cmidrule{3-6}
%       & & \raisebox{\dimexpr-1\normalbaselineskip-1\cmidrulewidth-1\aboverulesep}[0pt][0pt] {\shortstack[c]{Mobile \\ Seg. IoU $\uparrow$}}  & Prismatic & \multicolumn{2}{c}{Revoulute} \\
%       \cmidrule{4-6}
%       & & & Angle Err. $\downarrow$ & Angle Err. $\downarrow$ & Pos Err. $\downarrow$ \\
%      \midrule
%      \multirow{4}{*}{\shortstack[l]{Initial stage}}
%      & ScrewNet~\cite{} & X & X & X & X \\
%      & ANCSH~\cite{} & X & X & X & X \\     
%      \cmidrule{2-6}
%      & Ours$_{init}$ w/o contact & 0.69 & 0.05 & 28.70 & 0.05 \\
%      & Ours$_{init}$ w/ contact & 0.75 & 0.04 & 29.26 & 0.05 \\
%      \midrule
%      \multirow{2}{*}{\shortstack[l]{Final stage}}
%      & Ours$_{art}$ w/ contact & X & - & X & X \\
%      & Ours$_{final}$ w/ contact & 0.81 & - & 13.50 & 0.02 \\
%      \bottomrule
%     \end{tabular}
%     \label{tab:articulation}
% \end{table*}



\begin{table}[t]
    \small
    \centering
    \begin{tabular}{l|c|c|cc}
    \toprule
\raisebox{\dimexpr-1\normalbaselineskip-2\cmidrulewidth-2\aboverulesep}[0pt][0pt]{Method} & \multicolumn{1}{c|}{Geometry} & \multicolumn{3}{c}{Joint} \\
      \cmidrule{2-5}
      & \raisebox{\dimexpr-1\normalbaselineskip-1\cmidrulewidth-1\aboverulesep}[0pt][0pt] {\shortstack[c]{Mobile \\ Seg. IoU $\uparrow$}}  & Prismatic & \multicolumn{2}{c}{Revoulute} \\
      \cmidrule{3-5}
      & & Angle Err. $\downarrow$ & Angle Err. $\downarrow$ & Pos Err. $\downarrow$ \\
     \midrule
     ScrewNet~\cite{} & X & X & X & X \\
     ANCSH~\cite{} & X & X & X & X \\
     Ours & 0.75 & 0.04 & 29.26 & 0.05 \\
     Ours (art) & X & - & X & X \\
     Ours (art+moment) & 0.81 & - & 13.50 & 0.02 \\
     \bottomrule
    \end{tabular}
    % \vspace{-3mm}
    \caption{Quantitative results of articulation estimation.}
    % \vspace{-4mm}
    \label{tab:ablation}
\end{table}



% \begin{table*}[t]
%     \small
%     \centering
%     \begin{tabular}{l|c|c|cc}
%     \toprule
% \raisebox{\dimexpr-1\normalbaselineskip-2\cmidrulewidth-2\aboverulesep}[0pt][0pt]{Method} & \multicolumn{1}{c|}{Geometry} & \multicolumn{3}{c}{Joint} \\
%       \cmidrule{2-5}
%       & \raisebox{\dimexpr-1\normalbaselineskip-1\cmidrulewidth-1\aboverulesep}[0pt][0pt] {\shortstack[c]{Mobile \\ Seg. IoU $\uparrow$}}  & Prismatic & \multicolumn{2}{c}{Revoulute} \\
%       \cmidrule{3-5}
%       & & Angle Err. $\downarrow$ & Angle Err. $\downarrow$ & Pos Err. $\downarrow$ \\
%      \midrule
%      w/o contact & 0.69 & 0.05 & 28.70 & 0.05 \\
%      w/ contact & 0.75 & 0.04 & 29.26 & 0.05 \\
%      \bottomrule
%     \end{tabular}
%     % \vspace{-3mm}
%     \caption{Quantitative results of articulation estimation.}
%     % \vspace{-4mm}
%     \label{tab:ablation}
% \end{table*}



\begin{figure*}[t]
    \centering
    \resizebox{1.0\textwidth}{!}{
	\begin{tabular}
		{@{\hspace{0mm}}c@{\hspace{1mm}} @{\hspace{0mm}}c@{\hspace{1mm}} @{\hspace{0mm}}c@{\hspace{1mm}}
			@{\hspace{0mm}}c@{\hspace{1mm}} @{\hspace{0mm}}c@{\hspace{1mm}} @{\hspace{0mm}}c@{\hspace{0mm}}
		}
		
		Before & After & Contact region & ANCSH~\cite{} & Ours & Ours+contact \\
  
		\includegraphics[width=0.22\linewidth]{figs/test.png} &
		\includegraphics[width=0.22\linewidth]{figs/test.png} &
		\includegraphics[width=0.22\linewidth]{figs/test.png} &
		\includegraphics[width=0.22\linewidth]{figs/test.png} &
		\includegraphics[width=0.22\linewidth]{figs/test.png} &
		\includegraphics[width=0.22\linewidth]{figs/test.png} \\
		
	\end{tabular}
	}
	\caption{
    	\textbf{Ablations on contact region input.}
            \todo{}
	}
% 	\vspace{-3mm}
	\label{fig: ablation_contact}
\end{figure*}



\begin{figure*}[t]
    \centering
    \resizebox{1.0\textwidth}{!}{
	\begin{tabular}
		{@{\hspace{0mm}}c@{\hspace{1mm}} @{\hspace{0mm}}c@{\hspace{1mm}} @{\hspace{0mm}}c@{\hspace{1mm}}
			@{\hspace{0mm}}c@{\hspace{1mm}} @{\hspace{0mm}}c@{\hspace{0mm}}
		}
		
		Before & After & Contact region & Ours & Ours+art+moment \\
  
		\includegraphics[width=0.22\linewidth]{figs/test.png} &
		\includegraphics[width=0.22\linewidth]{figs/test.png} &
		\includegraphics[width=0.22\linewidth]{figs/test.png} &
		\includegraphics[width=0.22\linewidth]{figs/test.png} &
		\includegraphics[width=0.22\linewidth]{figs/test.png} \\
		
	\end{tabular}
	}
	\caption{
	    \textbf{Ablations on initial vs. final observations.} \todo{}
	}
% 	\vspace{-3mm}
	\label{fig: ablation_init_final}
\end{figure*}


\begin{figure*}[t]
    \centering
    \includegraphics[width=\textwidth]{figs/test.pdf}
    % \vspace{-5mm}
    \caption{
    \textbf{Qualitative result on virtual scene.} \todo{}}
    \label{fig: virtual}
\end{figure*}


\begin{figure*}[t]
    \centering
    \includegraphics[width=\textwidth]{figs/test.pdf}
    % \vspace{-5mm}
    \caption{
    \textbf{Qualitative result on real-world scene.} \todo{}}
    \label{fig: real_world}
\end{figure*}
